Deep Latent-Variable Models for Text Generation

Text generation aims to produce human-like natural language output for down-stream tasks. It covers a wide range of applications like machine translation, document summarization, dialogue generation and so on. Recently deep neural network-based end-to-end architectures have been widely adopted. The end-to-end approach conflates all sub-modules, which used to be designed by complex handcrafted rules, into a holistic encode-decode architecture. Given enough training data, it is able to achieve state-of-the-art performance yet avoiding the need of language/domain-dependent knowledge. Nonetheless, deep learning models are known to be extremely data-hungry, and text generated from them usually suffer from low diversity, interpretability and controllability. As a result, it is difficult to trust the output from them in real-life applications. Deep latent-variable models, by specifying the probabilistic distribution over an intermediate latent process, provide a potential way of addressing these problems while maintaining the expressive power of deep neural networks. This dissertation presents how deep latent-variable models can improve over the standard encoder-decoder model for text generation.

==> acknowledgements.tex <==
\thispagestyle{plain}
\chapter*{\Huge Acknowledgements}
First and foremost I would like to express my sincerest gratitude to my advisors Prof. Dr. Dietrich Klakow and Prof. Dr. Gerhard Weikum for their great supports of my PhD study. Their deep academic insights and rich knowledges helped me a lot in the research work during my PhD. More importantly, their attitudes and encouragement will be always inspiring to me in my future work. Besides, working with them, I also learned how to define, discover, address, present and publish my research works, which will be absolutely important in my future research works.
In addition, I would like to show my appreciation to Prof. Dr. Verena Wolf, Dr. Mathias Humbert and Prof. Dr. Akiko Aizawa, who kindly guided me through my initial stage of research work. They always encouraged me to explore some new ideas, selflessly shared their experience and provided high-quality feedbacks, which deeply influenced my understanding on good academic activity.
Thank you all for your time and effort for reviewing my work and providing valuable feedback.

In the following, I would like to thank people who I have collaborated with: Pascal Berrang, Prof. Dr. Satoshi Sekine, Hui Su, Yang Zhao, Prof. Dr. Kentaro Inui, Prof. Dr. Jun Suzuki, Prof. Dr. Vera Demberg, Ernie Chang, Liqiang Wang and Yafang Wang. I also learned a lot from you and growed a lot working with you, from your academic ability or personality. Besides, I would like to thank many other members (or former members) in the LSV group of Saarland University, including Youssef Oualil, Clayton Greenberg, Mittul Singh, Thomas Trost, Aditya Mogadala, David Ifeoluwa Adelani, Michael a. Hedderich, Marius Mosbach, Volha Petukhova, Thomas Kleinbauer, Dana Ruiter, Dawei Zhu, Alexander Blatt, Anupama Chingacham, Ali Davody, Fech Scen Khoo, etc. However, the people I would like to show appreciations are not only limited to the mentioned people, but all LST Saarland and D5 members in the MPI-Informatics. Thanks for your talents and hard working, maintaining excellent academic circumstance. Your every amazing presentations and discussions are memorable to me.

Next, I would like to thank our secretary Angelika Obree and system administrator Nicolas Louis. Thanks a lot for your careful and patient work. You always kindly reminded me of many important issues and gave me a lot of suggestions, which were of great for my life in Saarbrucken. Besides, I would like to thank IT service staff, for their work on providing a stable and wonderful environment. I would also like to thank Michelle Carnell and Susnne Vohl from the graduate school office who patiently helped me settle up in Saarbrucken and provided help through my first year of coursework. I am funded by the IMPRS-CS fellowship. The works I finished throughout my PhD phase have been supported by the DFG collaborative
research center SFB 1102, Research Grants Council of Hong Kong (PolyU 152036/17E, 152040/18E), the National Natural
Science of China under Grant No. 61602451, JSPS KAKENHI Grant Number JP19104418, AIRPF Grant Number 30AI036-8 and SFB 248 ``Foundations of Perspicuous Software Systems" (E2). I am very grateful to all the above generous support.

Finally, I would like to thank my parents. I could not have pursued my PhD without your supports and love.




==> fewshot/main.tex <==
\chapter[Fewshot Text Generation with Augmented Non-paired Text]{Fewshot Text Generation with Target-Text-Augmented Back Translation}
\label{chap: fewshot}

\lettrine[lines=3]{D}ata-to-text generation has seen a rise in the adoption of seq2seq learning. 
However, neural models are data-hungry and require massive amount of annotated data to be competitive.
In this work, we study the few-shot scenario where only limited annotations are available, and propose a GPT2-based target text augmentation~\footnote{The code to our seq2seq model and sample augmented data is attached as the supplementary material. Full version will be released. }to boost the seq2seq learning. Synthetic text are obtained through a two-step process of slot-value replacement and GPT2 generation to enrich the space of target text. Pseudo training pairs are then built from these through a combination of back translation and representation matching. On both the E2E and WebNLG benchmarks, we show this weakly supervised training paradigm is able to outperform fully supervised seq2seq models with less than $10\%$ of annotated data. By utilizing all training data, our model can boost the performance of standard seq2seq by up to 5 BLEU points, establishing a new state-of-the-art on both datasets.

\section{Introduction}
Neural data-to-text generation has been the subject of much recent research. The task aims at transforming source-side structured data into target-side natural language descriptions~\citep{reiter2000building}. While neural end-to-end systems afford the advantage of easy adaptability~\citep{wen2015semantically,lebret2016neural,wiseman2017challenges}, huge amount of data-text pairs are still necessary to perform
on par with their rule-based counterparts. 
This makes it less appealing since the high cost of annotating abundant data might even overweigh the efforts of designing a complex, and usually more robust, rule-based system. With this in mind, this work targets at the few-shot scenario where only few data are annotated. We 
aim to answer \emph{how we can make most utilize of the scarce annotations to push the limit of neural models}. Figure~\ref{fig:sample} illustrates the scenario.

\begin{figure}
  \centering
\includegraphics[width=1.\columnwidth]{sample.pdf}
\caption{ \small
\textbf{Few-shot scenario}: The model is expected to learn the data-to-text generation with only few data, among all, being labeled. The example is taken from the E2E dataset.}
\label{fig:sample}
\end{figure}
% delete plus sign
% change table only - attribute value pairs

Exploiting back-and-forth consistency has been the most successful technique for un/semi-supervised text generation with little parallel data~\citep{he2016dual,artetxe2017unsupervised,lample2017unsupervised}. A few works have applied it on data-to-text~\citep{schmitt2019unsupervised,qader2019semi,su2020towards}. However, they all assume the presence of vast unpaired instances in \emph{both the source and target sides}. 
%In the above data-to-text applications, the authors simply remove the parallelism but still use all the data and text instances. 
This, unfortunately, is seldom the case in real-world data-to-text applications since \emph{target-side text usually come only with data annotations}~\citep{chu2019meansum,mogadala2020integrating}. As Figure~\ref{fig:sample} shows, target text carry very restricted information defined by data schema and follow task-dependent requirement, obtaining high-quality, even if unpaired, target text is itself challenging.
%~\footnote{Mining target-side text from huge online resources is still possible, but requires significant engineering work of searching, filtering and reediting~\citep{agarwal2018char2char}, in contrast with tasks like machine translation (MT) where in theory arbitrary monolingual text can be used.}.

In this work, we study the effects of forth-and-back consistency when no additional target text are available. Interestingly, we find it still benefits the few-shot data-to-text \emph{using only unpaired source data} through encoder sharing. 
%The best performance is achieved when enforcing the consistency in all four directions. 
To allow for the maximum efficacy, we propose a simple yet effective way of augmenting the target-side text by pretrained language models (LMs). It consists of two steps: information augmentation by slot-value replacement and LM augmentation by GPT2 generation. The augmented text, together with the few annotations and unlabeled data are then passed through the back-and-forth consistency objective to explore the latent relationships between data and text. Unlike related text augmentation works~\citep{freitag2018unsupervised}, our proposal assumes little to no domain-dependent heuristics or handcrafted rules.

Besides, inspired by recent works of automatically extracting parallel sentences for machine translation by representation matching~\citep{artetxe2019margin,ruiter2019self,}, we align each augmented text to its most similar unlabeled data defined in their encoded vector space, and treat them as pseudo pairs for training. The quality of the pseudo pairs will gradually increase as the encoder becomes better, which can reciprocally facilitate the learning of the encoder.

On two data-to-text benchmarks  E2E~\citep{novikova2017e2e} and WebNLG~\citep{gardent2017webnlg}, we show our LM-augmented weakly supervised model succeeds on outperforming fully supervised seq2seq, though utilizing less than $10\%$ of the data annotations. It also outperforms previous works which \emph{further assumes access to all the ground-truth target-side text}. When trained with full data annotations, it is able to boost the model performance by up to 5 BLEU points, establishing a new state-of-the-art on both datasets. %Notably, all are achieved \emph{without relying on any domain-dependent heuristics or handcrafted rules}. 

Last but not least, we tried initializing our encoder-decoder with Bart~\citep{lewis2020bart}, a large-scale seq2seq model pretrained on huge online resources of plain text. The results show that our model can offer orthogonal improvement on top of Bart. In summary, this work makes the following contributions:
\begin{enumerate}
    \item We study on the few-shot data-to-text scenario where, unlike previous works, no further target-side text are available.
    \item We show for the first time that back-and-forth consistency can be combined with target text augmentation and outperforms standard seq2seq with less than 10\% data annotations.
    %\item Extensive ablation study is performed to understand the effects of each component in our proposed model.
    \item The proposed model is shown to be complementary with current seq2seq pretraining techniques, and can offer orthogonal improvements when combining both.
\end{enumerate}
\section{Related Work}
%Traditionally, data-to-text generation consists of modules that aim to select attributes and values from tables and verbalizing them into text \citep{reiter2000building,barzilay2005collective}. 
%Initially these approaches depend on heuristics to capture the data-to-text relationship, which can be non-trivial. On the other hand, 
%Recent neural approaches have achieved great success in data-to-text~\citep{wen2015semantically,lebret2016neural,wiseman2017challenges}.
%However, these neural systems require large-scale labeled data to perform on par with their rule-based counterparts \citep{van2018automated}.
The back-and-forth consistency objective has been ulitized in many text generation tasks like machine translation~\citep{artetxe2017unsupervised,lample2017unsupervised} and style transfer~\citep{prabhumoye2018style,subramanian2018multiple} to enable semi/un-supervised learning with few parallel data. \citet{schmitt2019unsupervised,qader2019semi,su2020towards} further applied this idea on data-to-text. Nonetheless, they all assume the existence of \emph{large-scale target-side text}, which, as we mentioned, is an unrealistic assumption for data-to-text.
 \citet{freitag2018unsupervised} proposes to reconstruct usable sequences re-written from data with rules for unsupervised data-to-text. 
Unfortunately, designing these rules require efforts similar to building a template-based system. 
\citet{budzianowski2019hello,chen2019few, peng2020few} tackles the few-shot challenge by finetuning a pretrained LM to incorporate prior knowledge from general-domain text or data-text pairs. We show our technique is complementary with them and can offer orthogonal improvements when combining both.

\section{Problem Formulation}
\label{sec:length}
We represent the data domain as \textit{D} and the text domain as \textit{T}. In our work, we do not restrict the format of the data. Each $d \in D$ can be a set of key-value pairs, as in Figure~\ref{fig:sample}, or in form of RDF triples as in \citet{gardent2017webnlg}. Each text $t \in T$ consists of a sequence of words.
In few-shot settings, we are assumed to have (1) $k$ labeled pairs $(D_L, T_L)$ and (2) A large quantities of unlabeled data $D_U$ where $|D_U| \gg k > 0$~\footnote{We force $k>0$ as we believe a reasonable generation system needs a least a few demonstrations of the annotation.}. This, we believe, is a more realistic setting as unlabeld data are usually abundant and also can be easily fabricated from predefined schema. Notably, we assume no access to outside resources containing in-domain text. The $k$ annotations are all we know about the target text.

\section{Approach}
To boost the seq2seq learning under this fewshot scenario, we start from the idea of encouraging back-and-forth consistency, which has been the most effective technique for semi/unsupervised text generation~\citep{he2016dual,artetxe2017unsupervised,lample2017unsupervised}. In the following section, we first elaborate on the idea of back-and-forth consistency~(\cref{sec: back-and-forth}), then explain how to address its shortcomings when applies to our scenario by combining it with target text augmentation~(\cref{sec: tt-aug}) and representation matching~(\cref{sec: rm}). Finally, \cref{sec: summary} makes a summary and presents the detailed algorithm.
\subsection{Back-and-forth Consistency}
\label{sec: back-and-forth}
The core idea of encouraging back-and-forth consistency is that starting from one sample in a domain, the model first maps it into the other domain, then maps it back~\citep{he2016dual}. It should come back to the original sample itself. Specifically, let $p_\theta(t|d)$ be the probability distribution to map a data $d$ to its corresponding text $t$, and $p_\phi(d|t)$ be the probability distribution to map text back to data. Starting from a data $d \in D$, its objective is:
\begin{equation}
\label{eq: dtd}
\begin{split}
    \max_{\phi}      \mathbb{E}_{d \sim p(D)}\log p_\phi(d|t');\;
    t' \sim p_\theta(t|d)
\end{split}
\end{equation}
which basically ensures the consistency in the direction of $d \rightarrow t' \rightarrow d$. Note that only $p_\phi$ is updated in this direction and $p_\theta$ serves only as as an auxiliary function to provide pseudo samples $t'$ from $d$. Though it is also possible to update $\theta$ at the same time through tricks like Gumbel-softmax or REINFORCE, we find it did not lead to better performance yet complicate the training. Similar observations are also found in \citet{lample2018phrase,he2020probabilistic,garcia2020multilingual}.

Similarly, starting from a text $t \in T$, the objective is to ensure the consistency in the direction of $t \rightarrow d' \rightarrow t$~\footnote{This direction is usually termed as \emph{back translation} in MT community~\citep{sennrich2016improving,lample2018phrase}}:
\begin{equation}
\label{eq: tdt}
\begin{split}
    \max_{\theta}      \mathbb{E}_{t \sim p(T)}\log p_\theta(t|d');\;d' \sim p_\phi(d|t)
\end{split}
\end{equation}
Finally, we further add two denoising autoencoding objectives on both the data and text sides:
\begin{equation}
\label{eq: ae}
    \max_{\theta,\phi} \mathbb{E}_{d \sim p(D), t \sim p(T)} \log p_\phi(d|\Tilde{d})p_\theta(t|\Tilde{t})
\end{equation}
where $\Tilde{d}$ and $\Tilde{t}$ are the corrupted $d$ and $t$. We use the same noise function as in \citet{lample2018phrase} which randomly permutes and pad a portion of the input. It can encourage the encoder to learn meaningful latent space by reconstructing the input itself~\citep{lample2018phrase}. 

Combining them, Figure~\ref{fig:directions} illustrates all the four directions of the back-and-forth objective.
\begin{figure}[t!]
  \centering
\includegraphics[width=\columnwidth]{directions.pdf}
\caption{\small Four directions of back-and-forth consistency. Gradients are backpropagated only through solid lines.}
\label{fig:directions}
\end{figure}
% split eq. 1 and 2
% only red line are trained, so change line color
% add tilda for noise representation, and remove gray
% add z according to drawing, add enc and dec for all diagrams
% dotted line
% remove number
% change arrow
% 


\begin{figure*}[t!]
  \centering
\includegraphics[width=0.85\textwidth]{gpt2.pdf}
\caption{\label{fig:augment}\small Target-Text Augmentation and Representation Matching. Each annotation first goes through information augmentation by slot-value replacement, then passed to GPT2 with iterative conditional generations. The augmented text are paired with the most similar data from the corpus with a threshold cutoff.}
\label{in_text_sample}
\end{figure*}




We use one shared encoder $Enc$ for both the data and text sides. Each data is flattened into a sequence as the text and fed into the same encoder. It gives the model an inductive bias to project similar data/text into surrounding latent space~\citep{chisholm2017learning}. We will show later that encoder sharing is essential for a good performance under the few-shot scenario. From the shared encoded space, two separate decoders $Dec_d$ and $Dec_t$ are utilized to decode $d$ and $t$ respectively~\footnote{We tried sharing the decoder as in \citet{johnson2017google} but find no improvement (see Table~\ref{tb:dir}).}.
\subsection{Target Text Augmentation}
\label{sec: tt-aug}
Our main goal is to decode text from a data, which involves only $Enc$ and $Dec_t$. Therefore, in the above four directions of objectives, $t \rightarrow d' \rightarrow t$ and $\Tilde{t} \rightarrow t$ are especially crucial since only the two involve the training of $Dec_t$. However, these two directions require sampling from $t \sim p(T)$, which, in our scenario, contains only $k$ annotations. This will greatly restrict the learning of $Dec_t$. To mitigate the paucity of $T$, we propose a pipeline approach to augment target text by (1) information augmentation and (2) LM augmentation.


\subsubsection{Information Augmentation}
\label{sec: info-aug}
We first consider a simple way of information augmentation by slot-value replacement. As many data values are exactly copied to the target text, these copied information can be easily detected and replaced with other values to enrich the information space of the target text. Specifically, we detect copied values for each annotation, then search on the whole data about the possible values of those slots. 
The copied parts are then randomly replaced with one of other possible values to form augmented text. This can be considered as a simplified version of traditional methods of template mining where key words are extracted to construct templates ~\citep{kondadadi2013statistical,oya2014template}. An example is shown in Figure~\ref{fig:augment}. Each text is augmented with 10 more distinct text or with all possible values being replaced.

The slot-value replacement is efficient to implement. However, it can only detect exactly copied values and augment text with the same combinatorial patterns as the fewshot annotations. To enrich the linguistic realizations of target text and enable new combinations of information, we further propose a LM augmentation approach by GPT2.

\subsubsection{LM Augmentation}
\label{sec: lm-aug}
 GPT2 is a language model pretrained on the huge WebText. It has demonstrated remarkable zero-shot multitask adaptability by simply feeding the input of each task into the LM and continuing to generate words~\citep{gpt2}. People have also also shown that GPT2 is able to improve classification tasks via in-domain text augmentation~\citep{papanikolaou2020dare,sun2020lamal}. We use a similar technique to first finetune GPT2 in the few-shot annotations~\citep{Wolf2019HuggingFacesTS}, then apply it to produce synthetic text through an iterative conditional generation process: With initial seeds being few-shot annotations (with information augmentation), LM iteratively conditions on previous output sentence to generate in-domain text~\footnote{We adopts the Top-$k$ random sampling with $k=2$ to encourage diversity and reduce repetition~\citep{gpt2}}. Each synthetic sentence is pruned if it (1) is shorter than 5 words or (2) contains only special tokens. The iterative generation is terminated when all tokens in the initial seeds are covered or reaches the maximum runs of 100. All the unpruned synthetic text are added into the space of $T$ to 
benefit the learning direction of $t \rightarrow d' \rightarrow t$ and $\Tilde{t}\rightarrow t$.
Figure~\ref{in_text_sample} depicts the generation process of GPT2.

In practice, obtaining clean in-domain text requires extreme efforts of designing heuristic rules. Nonetheless, the synthetic text from GPT2 make decent sense and can already provide useful signals to drive the learning process. 
%It can greatly enrich the semantic space of the target side to go beyond the original $k$ annotations. We show some examples of the synthetic text in Appendix C.

\subsection{Representation Matching}
    \label{sec: rm}
Apart from training under the forth-and-back consistency. We further consider matching each synthetic text into its most similar data and treating them as supplementary training pairs. Compared with the pseudo $d'$ obtained from back translation (Eq.~\ref{eq: tdt}), the matched data are extracted from the existing corpus and thereby is guaranteed to be clean. This can provide a much stabler training signal especially at the initial training stage~\footnote{In theory, as we can fabricate arbitrary possible data from the predefined schema and add to the corpus, we can always find one matched data for the target text.}.
%Previous works have shown that the cosine similarity of neural encodings can indicate the semantic similarity among sentences even in the initial training stage~\citep{sutskever2014sequence,espana2017empirical}. 
Previous works have used representation matching to automatically extract pseudo training pairs for machine translation~\citep{artetxe2019margin,ruiter2019self}. \citet{baziotis2019seq3,chu2019meansum} also demonstrate the representation similarity between input-output pairs can serve as a useful regularization for unsupervised text summarization. We adopt a similar idea to create pesudo pairs based on their cosine similarity on the representation space. The objective is:
\begin{equation}
\label{eq: rm}
\begin{split}
    \max_{\theta,\phi} \mathbb{E}_{t \sim p(T')} \mathbbm{1}_{cos(d^{\ast},t) > \varepsilon}(&\log p_\theta(t|d^{\ast}) \\ + &\log p_\phi (d^{\ast}|t));\\
    d^{\ast} = \argmax_{d \in D}\; &\text{cos}(d,t)
\end{split}
\end{equation}
where $T'$ is augmented text from LM and $\mathbbm{1}$ is the indicator function. The representation is defined as the mean pooling over the encoded space. $\varepsilon$ is a threshold. Pseudo pairs with a cosine similarity less than $\varepsilon$ will be discarded. Ideally, as the encoder improves, the pseudo pairs created by representation matching will make more sense, which can in turn benefit the training of the encoder. %Figure~\ref{in_text_sample} illustrates the idea of representation matching.

%\begin{figure}[t!]
%  \centering
%\includegraphics[width=1.0\columnwidth]{sim.pdf}
%\caption{\small Diagram of representation matching: parallel table-text pairs are sampled by signals from the model, where \textit{Sim} is the similarity function, and $t$ is the threshold. }
%\label{fig:cyclic}
%\end{figure}

\subsection{Summary}
\label{sec: summary}
Apart from the above unsupervised objective, on the few annotated data-text pairs, we can impose the supervised objective:
\begin{equation}
\label{eq: sup}
    \max_{\theta,\phi} \mathbb{E}_{d,t \sim p(D_L,T_L)} \log p_\theta(t|d) + \log p_\phi (d|t)
\end{equation}
where $(D_L,T_L)$ contains the $k$ data annotations. Putting all together, we summarize it in Algorithm~\ref{fewshot: alg}. In the training stage, we optimize the objectives of back-and-forth consistency, representation matching and supervised learning sequentially to maintain a constant ratio of signals from all sides.

\begin{algorithm}[tb]
   \caption{Few-shot Data-to-text}
   \label{fewshot: alg}
\begin{algorithmic}
   \STATE {\bfseries Input:} $D_U, (D_L, T_L)$
   \STATE Create $(D_a, T_a)$ by info augment (\cref{sec: lm-aug});
   \STATE $(D_L, T_L) \leftarrow (D_L, T_L) \cup (D_a, T_a)$;
   \STATE Create $T'$ by LM augment (\cref{sec: lm-aug});
   \STATE $T \leftarrow T_L \cup T'$;
   \REPEAT
   \STATE \textbf{Back-and-forth consistency:}
   \STATE Optimize by Eq.~\ref{eq: dtd} + Eq.~\ref{eq: tdt} + Eq.~\ref{eq: ae};
   \STATE \textbf{Representation Matching:}
   \STATE Optimize by Eq.~\ref{eq: rm};
   \STATE \textbf{Supervised Training:}
   \STATE Optimize by Eq.~\ref{eq: sup};
   \UNTIL{convergence}
\end{algorithmic}
\end{algorithm}

\section{Experiment Setting}
\label{sec:exp}
\paragraph{Data}
We conduct experiments on the E2E~\citep{novikova2017e2e} and WebNLG~\citep{gardent2017webnlg} datasets. E2E is a crowd-sourced dataset containing 50k instances in the restaurant domain. The inputs are dialogue acts consisting of three to eight slot-value pairs. WebNLG contains 25k instances describing entities belonging to fifteen distinct DBpedia categories. The inputs are up to seven RDF triples of the form \emph{(subject, relation, object)}. 

\paragraph{Config}
The model is implemented based on fairseq.
We use $600$-dimensional token embedding and Adam optimizer with initial learning rate at $0.0002$. 
Batch size is kept at $48$ with a dropout rate at $0.3$. 
We employ beam search with size $3$ for decoding and select
models based on BLEU-4 scores on the development set. The score is averaged over 10 random initialization runs.


%\paragraph{Evaluations.}
%For automatic evaluation on both datasets, we report degree of word-level overlap with human references in BLEU-4 \citep{bleu}, NIST~\citep{doddington2000nist}, ROUGE-L~\citep{lin2004rouge}, and METEOR~\citep{banerjee2005meteor}.
%For human-based evaluations \citep{belz2006comparing}, we perform \textit{intrinsic}\footnote{Evaluations in which humans rate given texts \citep{galliers1993evaluating}.} human evaluations with Amazon Mechanical Turk\footnote{\url{https://www.mturk.com/}} where eight subjects are shown texts generated by different systems \citep{coch1996evaluating}, and rate them based on \textit{fluency} on scale of $5$ similar to \citet{belz2006comparing}. Further, we manually count the coverage ratios on the E2E test set for selected attributes by matching the placeholders in delexicalized texts to input tables. We also count the number of missing attributes (\textit{miss}), and number of attributes incorrectly expressed in words (\textit{wrong}) on $30$ randomly sampled outputs \citep{duvsek2018findings,duvsek2020evaluating}.

\section{Results and Analysis}

\begin{table*}
  \small
  \centering
  \resizebox{1\textwidth}{!}{
  \begin{tabular}{lcccccccc}
    \toprule
    % \hline
    \multirow{2}{*}{Model} & \multicolumn{4}{c}{E2E - 10\%} & \multicolumn{4}{c}{E2E - 100\%} \\
    % \cline{2-9}
    \cmidrule(r){2-5}
    \cmidrule(r){6-9}
     & BLEU & NIST & METEOR & ROUGE-L & BLEU & NIST & METEOR & ROUGE-L \\
    %  \hline
    \cmidrule(r){1-1}
    \cmidrule(r){2-5}
    \cmidrule(r){6-9}
    SLUG & - & - & - & - & 66.19 & 8.61 & 44.54 & 67.72\\
    Seq2seq & 53.38 & 6.10 & 38.10 & 60.53 
    & 63.32 & 6.81 & 41.25 & 62.91 \\
    \citet{qader2019semi} & 58.10& 6.24 & 41.32 & 62.84 
    & 64.20 & 7.14 & 44.68 & 65.31 \\
    \citet{chen2019few} & 59.10 & 7.49 & 40.25 & 63.23
    & 63.72 & 7.76 & 40.25 & 66.23\\
    Proposed (LSTM) & 64.24  & 7.71 & 43.53 & 66.81 
    & 68.88  & 8.89 & 48.53 & 72.12\\
    Proposed (Bart) & \textbf{67.19}  & \textbf{7.95} & 
    \textbf{45.38} &
    \textbf{68.55} &
    \textbf{73.64} &
    \textbf{8.93} &
    \textbf{49.78} &
    \textbf{75.42}\\
    \midrule
    \midrule& \multicolumn{4}{c}{WebNLG - 10\%} & \multicolumn{4}{c}{WebNLG - 100\%} \\
    \cmidrule(r){2-5}
    \cmidrule(r){6-9}
    Model & BLEU & NIST & METEOR & ROUGE-L & BLEU & NIST & METEOR & ROUGE-L \\
    \cmidrule(r){1-1}
    \cmidrule(r){2-5}
    \cmidrule(r){6-9}
    Melbourne & - & - & - & - 
    & 44.93 & 8.98 & 36.58 & 60.40\\
    Seq2seq & 36.54 & 7.3 & 35 & 54.61
    & 44.60 & 8.49 & 38.23 & 59.67\\
    \citet{qader2019semi} & 38.66 & 7.81 & 34.1 & 56.95
    & 47.19 & 8.71 & 37.90 & 58.61\\
    \citet{chen2019few} & 39.40 & 7.84 & 37.25 & 56.23
    & 46.15 & 8.52 & 39.1 & 58.5\\
    Proposed (LSTM) & 43.75  & 8.29 & 33.58 & 58.49
    & 50.26  & 8.86 & 40.71 & 61.29\\
    Proposed (Bart) & \textbf{48.67}  & \textbf{7.19}
    & \textbf{36.80}
    & \textbf{61.62}
    & \textbf{54.69}
    & \textbf{9.43}
    & \textbf{44.58}
    & \textbf{63.72}\\
    \bottomrule
  \end{tabular}}  
\caption{\label{tb:comparison} \small Performance on E2E and WebNLG with 10\% and 100\% data. \citet{qader2019semi} utilizes all ground-truth unpiared target text while our proposed model only gets access to the fewshot data annotations.}
\end{table*}
In this section, we present experiment results and analysis. We first compare our model with other baselines on both datasets, then perform a set of ablation studies on the E2E dataset to see the effects of each component. Finally, we analyze how target text augmentation helps improves the model and include example outputs in the end.
\paragraph{Comparison with Other Models}
In Table~\ref{tb:comparison}, we compare our model with (1) seq2seq baseline, (2) back-and-forth consistency model as in \citet{qader2019semi}~\footnote{The author did not open-source their code. We reproduced their model based on our implementation. The results on 10k annotations matches their reports in the paper.} and (3) finetuned GPT2 model as in \citet{chen2019few}~\footnote{https://github.com/czyssrs/Few-Shot-NLG}. 
For all models, we try running with 10\% and 100\% annotations to see how they perform under different data sizes. Our model is implemented both with LSTM encoder-decoders, same as the seq2seq baseline for a fair comparison, and initialized with Bart, a pretrained powerful Transformer. Note that \citet{qader2019semi} further \emph{utilized all the ground-truth unpaired target text}, while the other models run only on the fewshot annotations.
We also include the results of \textbf{SLUG}~\citep{juraska2018deep} and \textbf{MELBOURNE}, the overall winner on automatic metrics in the E2E and WebNLG challenge respectively(both seq2seq-based). SLUG uses a heuristic slot aligner based on a set of handcrafted rules and combine a complex pipeline of data augmentation, selection, model ensemble and reranker.

The results show that our proposed model significantly improves over the baseline on both the fewshot and fully supervised setting. The improvement is more evident when only 10\% annotations are available, with a leap of 11 and 7 BLEU scores on E2E and WebNLG respectively. It also outperforms systems relying on task-dependent heuristics. When initialized with Bart, the performance can be further boosted, establishing new SOTAs on both datasets. In comparison, \citet{qader2019semi}, though with access to all target text, still underperforms our model with tangible margin. On the fully supervised setting, it brings little to no difference compared with the seq2seq baseline as no more extra data is incorporated in the training process. The finetuned GPT2 model helps on the fewshot setting, but its advantage also vanishes when all data annotations are available.

\begin{figure*}[ht]
  \centering
\includegraphics[width=0.9\textwidth]{few.pdf}
\caption{\small Model performance with varying number of data annotations. Our model with 10\% annotations outperforms the seq2seq model trained on $100\%$ pairs (dotted line) on both datasets. Shades are the sample standard deviation based on 10 runs of different model initializations. 
}
\label{fig:few}
\end{figure*}

In Figure~\ref{fig:few}, we draw the model performance with varying number of data annotations. All models are trained from scratch with 10 different random initializations and the standard deviation of the BLEU-4 score is visualized. We can see our model (LSTM-based), though with a relatively larger standard deviation due to the uncertainty of text augmentation sampling, still consistently outperforms other baselines significantly and even surpasses the fully supervised seq2seq model with less than 10\% of data annotations.
% single column
% add results for 1k datapoints 
% add one more line for other systems from shared task results 


\paragraph{Back-and-forth Consistency}
In Table~\ref{tb:dir}, we study how the four directions, input noise and parameter sharing affect the performance of back-and-forth-consistency. The experiments are conducted with 10\% annotations and \emph{no further unpaired target text are available}.
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c}

\small\textbf{Model/Share}  & \textbf{\small None}  & \textbf{\small Enc}   & \textbf{\small Dec} & \textbf{\small Both} \\ \hline
 \small \textbf{Supervised}                     & 53.20  & -    & -        & -     \\ %\hline
\textbf{+ $t \rightarrow d' \rightarrow t$}     & 53.19  & 53.28    & 53.17        & \textbf{53.29}    \\ %\hline
 \textbf{+ $d \rightarrow t' \rightarrow d$}    & 53.15  & \textbf{56.12}    & 53.49        & 56.07    \\ %\hline
  + $t \rightarrow t$                   & 53.74  & \textbf{56.39}    & 55.29        & 55.73      \\ %\hline
 + $d \rightarrow d$                    & 53.37  & \textbf{56.44}    & 56.09        & 56.11    \\
 + Noise                                        & 54.13  & \textbf{57.37}    & 56.59        & 57.04  \\
 + Bart                                         & 57.94  & \textbf{61.45}    & 57.61        & 59.91  \\\hline
\end{tabular}
}
\caption{\label{tb:dir}\small Ablation study for back-and-forth consistency (10\% annotations). BLEU-4 score is reported. Each line adds one condition on top of the previous one. \textbf{Supervised} is a supervised seq2seq baseline.}
\end{table}

As can be observed, adding the training direction $t \rightarrow d' \rightarrow t$ (aka. back translation) has little effects on top of the supervised seq2seq baseline. This is expectable since back translation is naturally designed to incorporate additional unpaired target text. When run only on the fewshot annotations, its power is very limited. The backward direction $d \rightarrow t' \rightarrow d$ is surprisingly useful when the encoder is shared between the data and text. Though this direction will not affect the text decoder at all, the improvement suggests the model can benefit a lot by simply structuring its encoded space and mapping aligned data-text to similar vector space. The autoencoding directions brings a little improvement. When combined with input noise, the performance further increases. This is similar to previous findings that denoising autoencoding is more helpful in inducing meaningful latent space~\citep{lample2018phrase} in comparison to simply learning to copy the original input. Initializing with Bart contributes to an improvement of roughly 3-5 BLEU points.

The results also suggest encoder sharing is important for the back-and-forth consistency objective to work in our fewshot setting. Decoder sharing, in contrast, makes little or even negative influence. This is kinda similar as in multilingual machine translation where sharing the decoder among languages might negatively interfere with the performance~\citep{johnson2017google}.
% limited improvements for t -> d' -> t
% more improvements for t' -> t
% slightly more for noise
% Bart 2 BLEU points 
% Dec for Bart would be slightly worse

\paragraph{Target Text Augmentation}
On top of the four-direction back-and-forth consistency training, we study the effects of target text augmentation in Table~\ref{tb:lmaug}. We compare our proposed info + LM augmentation with (1) random augmentation, where a random text from Wikipedia is sampled to the augmented text space, (2) unsupervised data augmentation~\citep{xie2019unsupervised} where target text are augmented with paraphrases of current annotations and (3) ground-truth augmentation with reference obtained from the left training corpus, which can serve as an upper bound of text augmentation techniques. We test the performance with 1\%, 5\%, 10\% and 20\% annotations to see the effects with varying number of supervisions.

As can be seen, the random augmentation even harms the model performance, suggesting reasonable in-domain text augmentation are necessary for the model improvement. UDA augmentation also makes rather little difference as it simply paraphrases the current available annotations but cannot bring any new information. The information augmentation by slot-value replacement helps improve a bit. When combined with LM, the performance can be further boosted, especially for lower-resource scenarios. The representation matching always helps lift the performance, with gains of up to 10 BLEU points. As expected, the benefit from text augmentation gradually vanishes as more annotations are collected, especially for datasets with relatively simple patterns as E2E.
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c}

\small\textbf{Text Augmentation}                  & \textbf{\small 1\%}  & \textbf{\small 5\%}   & \textbf{\small 10\% } & \textbf{\small 20\%} \\ \hline
 \small\textbf{None}   & 44.18  & 50.22   & 57.37   & 63.28     \\ \hline
Random                 & 41.30   & 49.62   &  57.71 & 62.79    \\ %\hline
UDA                    & 44.24  & 50.09   &  57.66 & 61.30    \\
Info                   & 45.63  & 52.22   &  58.80 & 63.22    \\ %\hline
+ LM                   & 48.67  & 53.53   & 59.04  & \textbf{64.78}    \\
Reference              & \textbf{55.33}  & \textbf{54.92}   & \textbf{59.11}  & 64.26      \\ \hline\hline
 Random (+RM)          & 42.32  & 50.10   & 58.53  & 63.29    \\
 UDA (+RM)             & 44.32  & 52.22   &  58.80 & 61.27    \\
 Info (+RM)            & 48.63   & 56.66   & 60.80  & 63.52    \\
 + LM (+RM)            & 53.18   & 59.12   & 64.24  & \textbf{65.38}  \\
 Reference (+RM)       & \textbf{62.74}   & \textbf{63.28}   & \textbf{64.93}  & 65.27 \\\hline
\end{tabular}
}
\caption{\label{tb:lmaug}\small Ablation study for text augmentation with varying number of annotations. LM augmentation outperforms random by a large margin and approaches, even outperforms sometimes, augmentation with ground-truth references.}
\end{table}
% Random < None 
% Reference > Rule+LM >> Rule >> None >> Random 
% +LM is correct, add based
% change to 1%, 5%, 10%, 20%

\begin{figure*}[t]
\centering
\small
\fbox{
\parbox{0.9\linewidth}{
\textbf{Data}:
\vspace{0.1cm}

[name] Blue Spice [eat type] restaurant [food] Chinese [area] city centre [family friendly] no [near] Rainbow Vegetarian Café  \\
\textbf{Reference}:
at the [city centre], there is a [restaurant] called the [Blue Spice].

\hrule
\vspace{0.1cm}
\textbf{seq2seq/info-aug}: Blue Spice restaurant near Rainbow Vegetarian Café has a \emph{5 star rating. prices start at £30}.
% \\
%\textbf{Rule}: The Cricketers coffee shop serves Japanese food.  It is situated near Raja Indian Cuisine at the riverside. It is not family-friendly.
 \\
\textbf{+LM-aug}: located near Rainbow Vegetarian Café is a Chinese theme eatery and restaurant called Blue Spice. It is in the city centre area.
 \\
}}
    \caption{\small Generation examples with different text augmentation techniques. Trained on 5 data annotations). The attribute combination of input data is unseen in the 5 annotations. Hallucinated contents are \emph{italitized}.
    }
    \label{fig: example}
\end{figure*}

\begin{figure*}[ht]
  \centering
\includegraphics[width=0.9\textwidth]{tokens.pdf}
\caption{\small \label{fig:unique} Additional number of decoded unique tokens (non-copied) and unique combinations of information on the testset with varying number of annotations.}
\label{fig:vocabulary}
\end{figure*}
% number of tokens not appearing in the source data
% only one bar chart: 10,100,500,1000 
%  < UDA < US 
% combine with the combination figure 


\begin{figure}[ht]
  \centering
\includegraphics[width=0.8\columnwidth]{sampling_selection.pdf}
\caption{\label{fig:epsilon} \small 
Performance of representation matching with varying $\varepsilon$. Best performance is achieved when $\varepsilon \approx$ 0.5.}
\label{fig:select}
\end{figure}
% change Epsilon to symbol 
% change scores to match 
Figure~\ref{fig:epsilon} further visualizes how the threshold $\epsilon$ affects the performance of representation matching. As can be observed, the best performance is achieved when $\epsilon \approx 0.5$. Setting it too small will bring too much noise and too large will be too strict for selection, so both negatively affects the model.

\paragraph{How text augmentation helps}
Intuitively the GPT2 augmentation is expected to impose new tokens and combination patterns to the fewshot annotations. To investigate whether this is the case, for the decoded text in the test phase, we count the number of unique tokens (excluding copied data values) and unique information combination patterns (attribute combinations in E2E). The results in Fig.~\ref{fig:unique} show that LM-augmentation indeed greatly enriches the vocabulary space, even doubling the generated unique tokens in low-resource scenarios. The same happens for new combination patterns. In contrast, info-aug cannot insert new tokens or combinations at all since all it does is replacing data values based on the same text annotation. UDA can impose new tokens by paraphrasing the annotations, but it hardly helps the model generalize to new combinations of information.

Figure~\ref{fig: example} shows a generation example with different text augmentation techniques. We train the systems in a toy setting with only 5 data annotations. We pick an input data with an unseen attribute combination to test if models can generalize correctly. Seq2seq and info-aug produce the wrong generation overfit to the information in the 5 training instances. With LM augmentation, it adapts to the new combination and connects information correctly.
\section{Conclusion}
We study few-shot data-to-text generation with only limited annotated data. We propose text augmentation with slot-value replacement followed by GPT2 generation. The augmented text, when combined with back-and-forth consistency and representation matching, is shown to help the model to generalize to unseen new tokens and patterns of token combinations. With less than 10\% annotations, it outperforms supervised seq2seq model trained on 100\% annotations and is extensible enough to be combined with pretraining techniques.

==> publications.tex <==
% \pagestyle{empty}
\definecolor{light}{gray}{0.65}
%
%%\section*{{\textcolor{light}{\Huge \bf Curriculum Vitae}}}
%\section*{{\Huge \bf Publications}}
%%\addcontentsline{toc}{chapter}{\protect\numberline{}{Curriculum Vitae}}   %% see book p. 176
%\vspace{0.02\textwidth}

\chapter*{\Huge{Publications}}

\vspace{1em}\noindent
{[6]} \textit{Improving Variational Encoder-Decoders in Dialogue Generation.}\\
\ul{Xiaoyu Shen}$^*$, Hui Su$^*$, Shuzi Niu, and Vera Demberg.\\
In Proc. of the AAAI Conference on Artificial Intelligence (\textbf{AAAI}), 2018.

\vspace{1em}\noindent
{[5]} \textit{Nexus Network: Connecting the Preceding and the Following.}\\
\ul{Xiaoyu Shen}$^*$, Hui Su$^*$, Wenjie Li, and Dietrich Klakow.\\
In Proc. of the Conference on Empirical Methods in Natural Language Processing (\textbf{EMNLP}), 2018.

\vspace{1em}\noindent
{[4]} \textit{Select and Attend: Towards Controllable Content Selection in Text Generation.}\\
\ul{Xiaoyu Shen}, Jun Suzuki, Kentaro Inui, Hui Su, Dietrich Klakow, Satoshi Sekine\\
In Proc. of the Conference on Empirical Methods in Natural Language Processing (\textbf{EMNLP}), 2019.

\vspace{1em}\noindent
{[3]} \textit{Improving Latent Alignment in Text Summarization by Generalizing the Pointer Generator.}\\
\ul{Xiaoyu Shen}, Yang Zhao, Hui Su, Dietrich Klakow.\\
In Proc. of the Conference on Empirical Methods in Natural Language Processing (\textbf{EMNLP}), 2019.

\vspace{1em}\noindent
{[2]} \textit{Neural Data-to-Text Generation via Jointly Learning the Segmentation and Correspondence.}\\
\ul{Xiaoyu Shen}, Ernie Chang, Hui Su and Dietrich Klakow\\
In Proc. of the Annual Meeting of the Association for Computational Linguistics (\textbf{ACL}), 2020.

\vspace{1em}\noindent
{[1]} \textit{Diversifying Dialogue Generation with Non-Conversational Text.}\\
Hui Su$^*$, \ul{Xiaoyu Shen}$^*$, Sanqiang Zhao, Xiao Zhou, Pengwei Hu, Rongzhi Zhong, Cheng Niu and Jie Zhou.\\
In Proc. of the Annual Meeting of the Association for Computational Linguistics (\textbf{ACL}), 2020.
